Chairs Can be Stood on: Overcoming Object Bias in Human-Object Interaction Detection

Detecting Human-Object Interaction (HOI) in images is an important step towards high-level visual comprehension. Existing work often shed light on improving either human and object detection, or interaction recognition. However, due to the limitation of datasets, these methods tend to fit well on frequent interactions conditioned on the detected objects, yet largely ignoring the rare ones, which is referred to as the object bias problem in this paper. In this work, we for the first time, uncover the problem from two aspects: unbalanced interaction distribution and biased model learning. To overcome the object bias problem, we propose a novel plug-and-play Object-wise Debiasing Memory (ODM) method for re-balancing the distribution of interactions under detected objects. Equipped with carefully designed read and write strategies, the proposed ODM allows rare interaction instances to be more frequently sampled for training, thereby alleviating the object bias induced by the unbalanced interaction distribution. We apply this method to three advanced baselines and conduct experiments on the HICO-DET and HOI-COCO datasets. To quantitatively study the object bias problem, we advocate a new protocol for evaluating model performance. As demonstrated in the experimental results, our method brings consistent and significant improvements over baselines, especially on rare interactions under each object. In addition, when evaluating under the conventional standard setting, our method achieves new state-of-the-art on the two benchmarks.

==> latex/3_bias.tex <==
\section{Object Bias Identification} \label{sec:bias}
% As is shown in previous research, the shortcut bias are generally from two respects: the unbalanced label distribution and the learning process which grasps such bias and amplify it~\cite{zhao2017menlikeshopping}.
% In this section, we analyze them separately to have a intuitive look at the object bias problem.
% In this section, we empirically study the \textit{object bias} problem in HOI detection.
The bias problem in HOI detection refers to predicting interactions based on the unbalanced training statistics under each object.
In the following, we demonstrate that the \textit{object bias} comes from two aspects: 
(1) the conditionally biased label distribution induced by object and 
(2) the biased model trained on the existing dataset.


% In this section, we utilize the HICO-DET~\cite{HORCNN_Chao2018WACV} dataset, which is currently the largest and commonly used in HOI Detection task to show some insights.
% We analyze the behavior of state-of-the-art two-stage and one-stage methods - SCG~\cite{zhang2021spatially_SCG_ICCV21} and CDN~\cite{zhang2021mining_CDN_NIPS21}, respectively. 

\subsection{Conditionally Biased Label Distribution}
% \input{latex/figures/objwise_dist}
% We utilize the HICO-DET~\cite{HORCNN_Chao2018WACV} dataset, which is currently the largest and commonly used in HOI Detection task to show some insights.
In HOI detection, where the task is usually to detect and classify \Triplet{human}{verb}{object} triplets, the most challenging and crucial part for interaction recognition is verb classification.
Denote the whole verb set as $\mathcal{V}$, the feasible verb set $\mathcal{V}_o$ for object $o$ is often a small fraction of all verbs, i.e. $\mathcal{V}_o \in \mathcal{V}$ and $|\mathcal{V}_o| < |\mathcal{V}|$.
Denote $p_o(v)$ as the verb distribution involved only verbs feasible with object $o$ and $p(v|o)$ the verb distribution conditioned on object $o$.
We further denote the support set of $p$ as $\mathcal{S}(p)$, then we have 
% $|\mathcal{S}(p(v)| = |\mathcal{V}| $ and 
$|\mathcal{S}(p_o(v))| = |\mathcal{S}(p(v|o))| = |\mathcal{V}_o|$.
However, as shown in Fig. ~\ref{fig:objbias31_dist}, even though both $p_v(o)$ and $p(v|o)$ are often long-tailed, they could be distinct from each other. 
% Fig. shows the verb distribution comparison between $p_o(v)$ and $p(v|o)$ under some objects in HICO-DET dataset.
For example, with the object \decorate{Microwave}, the most frequently associated verb is \decorate{operate}, while over the whole training set, \decorate{open} happens the most among all three feasible verbs.
Similar phenomenon can be observed for other objects.
We want to argue that this circumstance is pervasive in real-world.
Actually, we can \decorate{hold} a lot of objects which makes \decorate{hold} the most frequent verb over the HICO-DET dataset. 
But for some objects that are hold-able such as \decorate{Vase}, \decorate{hold} happens not that frequently.
%for example, we \decorate{sheep} is more often associated with \decorate{herd} and \decorate{bird} is more relative to \decorate{watch}.
Unfortunately, we observe such a commonplace may cause the model to learn \textit{object bias} without truly understanding the interactions, which is shown as follows.
% Similar, for all actions associated with the object \decorate{tie}, the most frequent action of the whole dataset is \decorate{hold}, while when conditioned on the it, it turns out \decorate{wear} to be the most related. 
% Such a long-tailed distribution under each object makes the model learn label statistics under each object, making the model learn \textit{object bias} for prediction.


% With the goal of the fitting the training set, a model is expected to learn dataset statistics as a type of shortcut bias.
% Nonetheless, in HOI detection, where the interaction recognition is always achieved by object classification and action classification, the dataset statistics under each object is often distinct from the global one.


\subsection{Biased Model Exploration}
% In this task, the verb recognition is often formulated as a multi-label classification problem.
To figure out how model suffers from bad performance, we study the behavior of the state-of-the-art model SCG~\cite{zhang2021spatially_SCG_ICCV21} on HICO-DET test set.
Denote $\hat{y}(v|o)$ as the score distribution of the output conditioned on object $o$ and $y(v|o)$ as the ground truth label distribution.
We adopt Jensen-Shannon Divergence as distance metric $D$ between distributions and visualize the distances on four objects in Fig.~\ref{fig:model_output}.
We observe that $\hat{y}(v|o)$ is closer to $p(v|o)$ than $p_o(v)$, indicating the model is learning object-conditional bias, rather than the global distribution statistics.
Besides, $\hat{y}(v|o)$ is much closer to $p(v|o)$ than the ground-truth distribution $y(v|o)$, suggesting the model is actually memorizing the training set object-conditional statistics, instead of truly understanding the interactions on the test set.
This phenomenon shows the unbalanced conditional label distribution is a key factor for the \textit{object bias problem}, which necessitates to alleviate the conditional label distribution unbalance. 
% Besides, the excessively large distance between 
% output does not understand the test set information .
% on application, we study the distance between output score $\hat{y}_o(v)$ on object and  for each object
% two types of error in multi-label classification - false positive and false negative. 
% In Fig.~\ref{fig:model_output}, we show the behavior of the state-of-the-art method SCG~\cite{zhang2021spatially_SCG_ICCV21} on HICO-DET test set.
% We observe that the false positive error are mainly concentrated on the classes that have more positive samples while false negative error are on those with less positive samples.
% This phenomenon is generally aligned with the object-conditional label distribution $p(v|o)$: the classes with more positive samples are assigned high scores while those with less positive samples are assigned with low ones, whatever the ground-truth is.
% This circumstance indicates the model often makes predictions based on the \textit{object bias}, instead of truly understanding the relationship between human and object, thereby affecting the performance and generalization of these methods.
% More illustrations can be found in our supplementary material.

==> latex/figures/ablation_read.tex <==
\begin{table}[!t]
    \centering
    \caption{\label{table:ablation_write_strategy}
        Comparison of different read and write strategies for EOM on HICO-DET dataset (with Detector dre-trained on MS-COCO).
    }
    \adjustbox{}{
    \begin{tabular}{l|ccc}
    \toprule
    Variant       &   \textbf{Full}    &   \textbf{Rare}    & \textbf{Non-Rare} \\
    \midrule
    Baseline                 &   20.99   &   16.30   &  22.40      \\
    \midrule
    Random Write             &   19.64    &   16.04    &   20.71       \\
    Random Read              &   19.66    &   15.42    &   20.92       \\
    Without Obj Splitting    &   20.16     &  16.96    &  21.12       \\
    Full (Ours)              &  \textbf{21.50}    &   \textbf{17.59}    &   \textbf{22.67}           \\
    \bottomrule
    \end{tabular}}
\end{table}

==> latex/figures/ablation_write.tex <==
\begin{table}[!t]
    \centering
    \caption{\label{table:ablation_write_strategy}
        Comparison of different write strategy for memory bank on HICO-DET dataset.
    }
    \adjustbox{}{
    \begin{tabular}{lccc}
    \toprule
    Method                                  &   Full    &   Rare    & Non-Rare \\
    \midrule
    Baseline                                        &   0.00    &   0.00    &   0.00    \\
    Random Write                                    &   23.53   &   8.29    &   35.36   \\
    Global Write                                    &   0.00    &   0.0     &   0.00    \\
    \midrule
    Weight Age  Only                                &   23.40   &   8.01    &   35.34   \\
    Weight Head Only                                &   25.29   &   9.85    &   37.27   \\
    Age + Head                                      &   0.00    &   0.0     &   0.0     \\
    % \midrule
    % SCG*~\cite{zhang2021spatially_SCG_ICCV21}&   0.0     &   0.0     &   0.0     \\
    % SCG + Ours                              &   0.0     &   0.0     &   0.0     \\
    \bottomrule
    \end{tabular}}
\end{table}

==> latex/figures/jsd.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth, trim=2 25 30 6, clip]{latex/images/objectbias-3_2b.pdf}
    \caption{\label{fig:jsd}
     The Jensen-Shannon divergence~\cite{lin1991jsd} is utilized to compute the distribution distance.
     Note that the values are increased 100x for better illustration.
    }
\end{figure}


==> latex/figures/model_output.tex <==
\begin{figure*}[ht]
    \vspace{-15pt}
    \centering
    \includegraphics[width=1.0\textwidth, trim=0 5 35 0, clip]{latex/images/objectbias-32new.pdf}
    % \vspace{-2em}
    \caption{\label{fig:model_output}
    The model output analysis of SCG~\cite{zhang2021spatially_SCG_ICCV21} on HICO-DET~\cite{HORCNN_Chao2018WACV} test set with four objects.
    We show the difference between conditional training distribution $p^{train}(v|o)$, averaged model output $\hat{y}(v|o)$ and ground-truth conditional verb distribution $p^{test}(v|o)$.
    % (b) The Jensen-Shannon divergence~\cite{lin1991jsd} is utilized to compute the distribution distance.
    % Note that the values are increased 100x for better illustration.
    % We observe the model output $\hat{y}_o$ for object $o$ is closer to the global 
    % Train means the verb ratio on the training set while SCG-FP and SCG-FN means the average error of false positive and false negative made by SCG, respectively.
    % The verbs are sorted according to their ratio in the training set and each row is normalized by the number of interactive human-object pairs associated with the object.
    % Note that the summation of each row can be great than one in the multi-class setting.
    % For both objects, the false positive error are concentrated on frequently positive classes while false negative error are on frequently negative classes.
    % This phenomenon indicates the are learning the \textit{object bias} by following the dataset statistics contiditioned on the object.
    }
    \vspace{-30pt}
\end{figure*}


==> latex/figures/quali.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\columnwidth, trim=0 0 0 0, clip]{latex/images/objectbias-Quali_short(8).pdf}
    % \vspace{-2em}
    \caption{\label{fig:quali}
    % Examples of qualitative results from HICO-DET test set.
    % The tag in the first row shows the ground-truth interaction while in the second row the tag shows the false positive interaction predicted by the baseline model.
    % Involved verbs are \textbf{bold}.
    % Our method can correct both False Negative and False Positive errors.
    % More results can be found at supplementary material.
    % Zoom in for details.
    False negative (top two) and false negative (bottom two) instances from the SCG baseline on HICO-DET test set.
    For each instance, the $p^{train}(v|o)$ is also shown, where involved verb is bold.
    }
    \vspace{-1em}
\end{figure}

